Robust Finite-time Stabilization of Linear Systems with Limited State Quantization

This paper investigates the robust asymptotic stabilization of a linear time-invariant (LTI) system by a static feedback with a static state quantization. It is shown that the controllable LTI system can be stabilized to zero in a finite time by means of a nonlinear feedback with a quantizer having a limited (finite) number of values (quantization seeds) even when all parameters of the controller and the quantizer are time-invariant. The control design is based on generalized homogeneity. A homogeneous spherical quantizer is introduced. The static homogeneous feedback is shown to be local (or global) finite-time stabilizer for the linear system (dependently of the system matrix). The tuning rules for both the quantizer and the feedback law are obtained in the form of Linear Matrix Inequalities (LMIs). The closed-loop system is proven to be robust with respect to some bounded matched and vanishing mismatched perturbations. Theoretical results are supported by numerical simulations. \

==> external.tex <==
{\begin{comment}
\begin{remark}\label{rmk:hom}
Since $\mathfrak{q}_{\pi_\dn}$ is dilation invariant, by property \eqref{eq:A_B_d}, for any $s\in\mathbb{R}$,  the system \eqref{eq:f_q}, \eqref{eq:u_c_2}  has \[
A\dn(s)x + BK\mathfrak{q}_{\pi_\dn}(\dn(s)x)=
     e^{-s}\dn(s)(Ax + BK\mathfrak{q}_{\pi_\dn}(x)).
\]
It implies that  \eqref{eq:f_q}, \eqref{eq:u_c_2}  is $\dn$-homogeneous of degree $-1$.
\end{remark}

\begin{remark}
For the controlled chain of integrator: \vspace{-2mm}
$$A=\left(\begin{smallmatrix} 0 & 1 & 0 & ...  & 0 & 0\\ 0 & 0 &1 & ...& 0 & 0\\
... & ... & ... & ... & ... & ...\\
0 & 0 & 0 & ... & 0 & 1\\
0 & 0 & 0 & ... & 0 & 0\\
\end{smallmatrix}\right), \quad B=\left(\begin{smallmatrix} 0  \\ 0\\
... \\
0 \\
1\\
\end{smallmatrix}\right), \vspace{-2mm}
$$
the dilation $\dn$ is diagonal, and the system \eqref{eq:f_q}, \eqref{eq:u_c_2} is globally finite-time stable with finite static quantization.
\end{remark}
For a linear plant with a homogeneous open-loop system, as discussed in Remark \ref{rmk:hom}, the closed system under quantized state feedback remains homogeneous, ensuring global finite-time stabilization with finite static quantization. The subsequent section addresses nonhomogeneous open-loop plant stabilization.


\subsection{Stabilization of non-homogeneous LTI system}
 
In state feedback control, for a nonhomogeneous matrix $A$, controllability ensures the existence of a linear state feedback gain $K_0x$, making $A_0 = A + BK_0$ homogeneous. Consequently, the design of homogeneous feedback is based on the system $(A_0, B)$. For a general linear plant, the system with feedback $u_{\text{hom}}(\mathfrak{q}_{\pi_\dn}(x))$ is design based Theorem \ref{thm:limited_data} with system $(A_0, B)$ can be represented as:
\begin{equation}
\dot{x} = A_0x + BK\mathfrak{q}_{\pi_\dn}(x) - BK_0x. \label{eq:nh_1}
\end{equation}
Since $\|x\|$ tends to zero as $\|x\|_\dn$ tends to zero, and $\|x\|$ tends to infinity as $\|x\|_\dn$ tends to infinity, the closed-loop system \eqref{eq:nh_1} is \textit{locally uniformly finite-time stable}.

%Stabilization with finite static quantization of a continuous-time linear plant into a neighborhood of the origin has been addressed in \cite{ferranteTAC2015} and \cite{wang2018Aut}. Then, for states within any compact set, stabilization with finite static quantization can be achieved by integrating the proposed homogeneous approach with the mentioned practical stabilization method.

On the other hand, if the linear state feedback $K_0x$ is replaced by quantized state feedback $K_0\tilde{\mathfrak{q}}(x)$, where $\tilde{\mathfrak{q}}:\mathbb{R}^n\mapsto\tilde{\mathcal{Q}}\subset\mathbb{R}^n$ is a quantizer on $\mathbb{R}^n$, the system can be represented as:
\begin{equation}
\dot{x} = A_0x + BK\mathfrak{q}_{\pi_\dn}(x) + BK_0(\tilde{\mathfrak{q}}(x) - x). \label{eq:nh_2}
\end{equation}
Since $G_\dn B = B$, according to Corollary \ref{cor:1}, if there exists a sufficiently small $\tilde{\kappa} > 0$ such that $\|\tilde{\mathfrak{q}}(x) - x\| \leq \tilde{\kappa}$ for all $x \in \mathbb{R}^n\setminus \{\boldsymbol{0}\}$, then the system \eqref{eq:nh_2} is \textit{globally uniformly finite-time stable}. In this case, while the quantization number of $\tilde{\mathfrak{q}}$ tends to infinity as $x$ tends to infinity, finite static quantization can guarantee finite-time stability for states within any compact set.




If we consider the linear state feedback as $K_0x$ satisfying uniform quantization, i.e., $\|K_0x - K_0\mathfrak{q}(x)\|\le \tilde{\delta}$, then, for a sufficiently small $\tilde{\delta}$, the closed-loop system can be represented as:
\[
\dot{x} = A_0x + BK\mathfrak{q}_{\pi_\dn}(x) + K_0(\mathfrak{q}(x)-x).
\]
In this case, the finite-time stability of the system with finite static quantization can be extended to almost global.
\end{comment}

